Towards Fast, Memory-based and Data-Efficient Vision-Language Policy

Vision Language Models (VLMs) pretrained on Internet-scale vision-language data have demonstrated the potential to transfer their knowledge to robotic learning. However, the existing paradigm encounters three critical challenges: (1) expensive inference cost resulting from large-scale model parameters, (2) frequent domain shifts caused by mismatched data modalities, and (3) limited capacity to handle past or future experiences. In this work, we propose LiteVLP, a lightweight, memory-based, and general-purpose vision-language policy generation model. LiteVLP is built upon a pre-trained 1B-parameter VLM and fine-tuned on a tiny-scale and conversation-style robotic dataset. Through extensive experiments, we demonstrate that LiteVLP outperforms state-of-the-art vision-language policy on VIMA-Bench, with minimal training time. Furthermore, LiteVLP exhibits superior inference speed while maintaining exceptional high accuracy. In long-horizon manipulation tasks, LiteVLP also shows remarkable memory ability, outperforming the best-performing baseline model by 18.8%. These results highlight LiteVLP as a promising model to integrating the intelligence of VLMs into robotic learning.

==> authors.tex <==
\author{Sungwon Han\thanks{Equal contribution to this work.}\textsuperscript{\rm ~~1}~~~Sungwon Park\footnotemark[1]\textsuperscript{\rm ~~1}~~~Fangzhao Wu\textsuperscript{\rm 2}~~~Sundong Kim\textsuperscript{\rm 3} \\ Bin Zhu\textsuperscript{\rm 2}~~~Xing Xie\textsuperscript{\rm 2}~~~Meeyoung Cha\textsuperscript{\rm 4,1} \\
\textsuperscript{\rm 1} KAIST 
\hspace{0.3cm} \textsuperscript{\rm 2} Microsoft Research Asia \hspace{0.3cm} 
\textsuperscript{\rm 3} GIST
\hspace{0.3cm} \textsuperscript{\rm 4} Institute for Basic Science 
%\small{\{psw0416, lion4151, danu, seunghoon.hong\}@kaist.ac.kr ~~\{sundong, shaun01, mcha\}@ibs.re.kr}
}



\if 0
\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}
\fi

==> table/3_multi_vs_single.tex <==
\begin{table}[!h]
\centering
\scalebox{0.9}{
\begin{tabular}{l|c|ccc|c}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Noise} & L1 & L2 & L3 & Avg Performance \\
                 &   & (\%) & (\%) & (\%) &  Drop(\%) \\\midrule
    \multi & 0 & 83.1 & 81.5 & 77.5 & - \\
    \single & 0 & 84.2 & 78.1 & 75.4 & - \\\midrule
    \multi & 0.2 & 76.5 & 78.5 & 70.0 & \textbf{4.2(5.3\%$\downarrow$)} \\
    \single & 0.2 & 77.7 & 75.4 & 70.0 & 6.3(7.8\%$\downarrow$) \\
    \multi & 0.5 & 76.2 & 75.8 & 65.4 & \textbf{6.8(8.6\%$\downarrow$)} \\
    \single & 0.5 & 70.4 & 65.8 & 60.8 & 15.0(18.6\%$\downarrow$) \\
    \multi & 0.8 & 75.4 & 75.0 & 64.6 & \textbf{7.6(9.6\%$\downarrow$)} \\
    \single & 0.8 & 66.5 & 63.5 & 58.3 & 17.9(22.2\%$\downarrow$)\\\bottomrule
    \end{tabular}}
\caption{\textbf{Performance of our method with different noise levels in object detection results.} The evaluations of performence drop of our two mode of 
image inputs, when varing noise levels(0, 0.2, 0.5) is added to the object detection results.}
\label{Tab:multi vs single}
\end{table}
